A tumor growth model with autophagy: the reaction-(cross-)diffusion system and its free boundary limit

In this paper, we propose a tumor growth model to incorporate and investigate the spatial effects of autophagy. The cells are classified into two phases: normal cells and autophagic cells, whose dynamics are also coupled with the nutrients. First, we construct a reaction-(cross-)diffusion system describing the evolution of cell densities, where the drift is determined by the negative gradient of the joint pressure, and the reaction terms manifest the unique mechanism of autophagy. Next, in the incompressible limit, such a cell density model naturally connects to a free boundary system, describing the geometric motion of the tumor region. Analyzing the free boundary model in a special case, we show that the ratio of the two phases of cells exponentially converges to a ``well-mixed" limit. Within this ``well-mixed" limit, we obtain an analytical solution of the free boundary system which indicates the exponential growth of the tumor size in the presence of autophagy in contrast to the linear growth without it. Numerical simulations are also provided to illustrate the analytical properties and to explore more scenarios.

==> neumann_arxiv.tex <==
%\documentclass[ms.tex]{subfiles}

\begin{document}
	
\section{Numerical simulations with Neumann boundary condition}\label{sc:Neumann}

In this section we consider a cell density model for tumor growing in a bounded domain $\Omega\subset\mathbb{R}^n$, which can be seen as a modified version of the PDE system \eqref{model:PDE-systems} with the Neumann boundary condition. We perform numerical simulations to study this model with more complicated settings than those in Section \ref{sc:math-proof} and \ref{sc:auto}. Here we allow the transition rates $K_1,K_2$ to depend on the nutrient concentration, the formation of necrotic core and the dynamical boundary condition for the nutrient concentration $c$.

\subsection{Setting of the Neumann problem}
We extend the cell density model \eqref{model:PDE-systems} to consider a tumor living in a bounded domain $\Omega\subset\mathbb{R}^n$. Since there shall be no flux of density going into or out of the domain, we have
\begin{equation*}
n_i\frac{\p p}{\p \mathbf{n}}=0,\quad x\in\p\Omega,\ t>0,\ i=1,2,
\end{equation*}where $\mathbf{n}$ is the outer normal vector of $\p\Omega$.  For motion of nutrients we consider \eqref{eq:model-c} with $\epsilon=1$ and a Neumann boundary condition denotes the input nutrient flux from the boundary. Precisely, we consider the following system:
\begin{spacing}{1.3}
	\begin{equation}\label{model:PDE-systems-Neumann}
	\begin{cases}
	\frac{\partial n_1}{\partial t}-\Div(n_1 \nabla p)=G(c)n_1-K_1(c)n_1+K_2(c)n_2,\quad x\in\Omega, t>0.\\
	\frac{\partial n_2}{\partial t}-\Div(n_2 \nabla p)=(G(c)-D)n_2+K_1(c)n_1-K_2(c)n_2,\quad x\in\Omega, t>0.\\
	n_i\frac{\p p}{\p \mathbf{n}}=0,\quad x\in\p\Omega,\ i=1,2.\\
	p=\frac{\gamma}{\gamma-1}(n_1+n_2)^\gamma,\ \gamma>1.\\
		\frac{\p c}{\p t}-\Delta c+ \psi(c)(n_1+n_2)=an_2,\quad x\in\Omega, t>0.\\
\frac{\p c}{\p \mathbf{n}}=-\lambda(t),\quad x\in\p\Omega,\ t>0,\\
	%-\Delta c+ \psi_1(c)n_1+\psi_2(c)n_2=0,\ \Omega(t)\\
	%c=c_B\ \p\Omega(t).
	\end{cases}
	\end{equation}\end{spacing}Here $\lambda(t)\geq0$ denotes the input of nutrients from the boundary. System \eqref{model:PDE-systems-Neumann} is completed with non-negative initial values for $n_1,n_2,c$. We remark that porous media type tumor growth models for two species with Neumann boundary condition, without nutrients, have been considered in literature (e.g., \cite{bertsch2010free,bertsch2012nonlinear,price2020global}).

As before the parameters satisfy \eqref{ap-1Da}$\sim$\eqref{ap-3psi}. In this section we allow $K_1(c),K_2(c)$ to vary with the concentration of nutrients, in contrast to Assumption \ref{as:constants}. Spatial heterogeneity in both total density $n$ and the density fraction $\mu$ arises from hetergenuous nutrients availability. Also, in the middle of the tumor a necrotic core may form due to the lack of nutrients. For example, see Figure \ref{fig:s5f1} where we plot the density of total cells $n$ and autophagic cells $n_2$ in one dimension with $\gamma=2$ and $\gamma=40$. %One can also see when $\gamma$ is small, the density looks more homogeneous and smoother.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.9\linewidth]{s5f1}
	\caption{Densities of all cells $n$ and of autophagic cells $n_2$ for $\gamma=2,40$ at $T=20$. Solid line: the total density $n$. Dashed line: the density of autophagic cells $n_2$. Plot at $T=20$. Parameters: $G(c)=c-\delta$ with $\delta=0.1$. $\psi(c)=c$. $D=0.5,a=0.5$. Transition rates satisfies $K_1(c)=k_{1,\max }\frac{\omega^{4}}{\omega^{4}+c^{4}},K_2(c)=k_{2,\max }\frac{c^{4}}{\omega^{4}+c^{4}}$ as in \eqref{eq:k1k2hull}, with $k_{1,\max}=k_{2,\max}=3,\omega=0.5$.}
	\label{fig:s5f1}
\end{figure}
\subsection{Numerical simulation}
\subsubsection{Parameters for numerical simulation}
 We carry out numerical simulations in a one-dimensional symmetric domain $\Omega=[-5,5]$. We adapt the numerical scheme in \cite{liu2018accurate} to treat the Neumann problem, with spatial grid length $\Delta x=0.04$ and time step $\Delta t=0.002$. The description of the numerical scheme is in Appendix \ref{app:num}.
 
 For the net growth rate $G(c)$ and the nutrient consumption rate $\psi(c)$ we choose the following forms unless otherwise specified:
\begin{equation}\label{eq:simple-G}
G(c)=c-\delta,\quad\psi(c)=c,
\end{equation}where $\delta>0$ is the death rate of normal cells.

For transition rates $K_1(c),K_2(c)$, we consider the following hull functions as in \cite{jin2014mathematical-autophagy}:
\begin{equation}\label{eq:k1k2hull}
\begin{aligned}
K_1(c)=k_{1,\max }\frac{\omega^{4}}{\omega^{4}+c^{4}},\\K_2(c)=k_{2,\max }\frac{c^{4}}{\omega^{4}+c^{4}}.
\end{aligned}
\end{equation}Here $k_{1,\max },k_{2,\max}>0$ can be used to adjust the magnitude of $K_1,K_2$. And $\omega>0$ reflects the scale of the concentration of nutrients $c$. Note that \eqref{eq:k1k2hull} satisfies $K_1'(c)<0,K_2'(c)>0$.

For the relation between $n$ and $p$ \eqref{eq:intro-p}, we choose $\gamma=40$.

Initially we let all cells be normal cells, i.e., the density fraction $\mu=1$. And set the pressure $p$ to be
\begin{equation*}
p(x,0)=\begin{cases}
1-\frac{\cosh x}{\cosh R},\quad |x|<R,\\0,\quad |x|\geq R,
\end{cases}
\end{equation*}which is a special case of \eqref{eq:ana-p} when $\mu=1$. We choose $R=4$ and recover the total density $n$ from \eqref{eq:intro-p}. For nutrients initially we set 
\begin{equation}\label{eq:init-c}
c(x,0)\equiv 1,\quad\forall x\in\Omega,
\end{equation}which is relatively sufficient.
\subsubsection{Autophagy helps survivability}

It is known that autophagy promotes cells survival under nutrient depletion. Experiments on yeasts have shown that cells with defective autophagy dramatically reduce their survivability under starvation while wild type cells maintain survival under the same condition \cite{thumm1994isolation}, whose experiment data has been fitted by the ODE model \cite{jin2014mathematical-autophagy}. This phenomenon is also observed in tumor growth \cite{lorin2013autophagy}.

In this model, $k_{1,\max}$ in \eqref{eq:k1k2hull} can be interpreted as the ability of autophagy. Since $K_1(c)$ is proportional to $k_{1,\max}$, when $k_{1,\max}$ is bigger, normal cells will change into autophagy cells with a faster rate. This results in a larger ratio of autophagic cells, at least heuristically, or in the simple case when the extra death rate $D=0$. 

Our goal in this subsection is to study the effects of autophagy under nutrient depletion by numerically simulating the Neumann problem \eqref{model:PDE-systems-Neumann} with different $k_{1,\max}$ under two kinds of nutrient input $\lambda(t)$.

First we consider the case when the nutrient input is constant in time, i.e., $\lambda(t)\equiv\lambda_0$. While initially the nutrient is sufficient \eqref{eq:init-c}, the nutrient input $\lambda(t)$ we choose is relatively small such that it is insufficient in the long term. From the evolution of total population $\int_{\Omega}n(x,t)dx$ in time (Figure \ref{fig:autohelp1} Left) one can see in a small initial period when the nutrient is sufficient, different $k_{1,\max}$ show little influence, while when the nutrient is no longer sufficient as time evolves, cells with higher $k_{1,\max}$ maintains a higher population, which is consistent with the ODE model in \cite{jin2014mathematical-autophagy}. Spatially in the graph of total density $n$ at a fixed time (Figure \ref{fig:autohelp1} Right), cells with higher $k_{1,\max}$ have a larger density as well as a smaller radius of necrotic core.
\begin{figure}[H]
	\begin{subfigure}{.5\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{s52f2}
		%\caption{}%Time evolution of total population $\int_{\Omega}n(x,t)dx$}% under different $k_{1,\max}$}
		%\label{fig:s52f2}
	\end{subfigure}
	\begin{subfigure}{.5\linewidth}
	\centering
 \includegraphics[width=0.9\linewidth]{s52f1}
%\caption{}%Graph of total density $n$ at $t=40$. Legend is the same as in (a)}
%		\label{fig:s52f1}
	\end{subfigure}
\caption{Left: Evolution of the total population $\int_{\Omega}n(x)dx$. Right: Plots of total density $n$ with different $k_{1,\max}$. We only show the total density $n$ in a half of the domain thanks to symmetry.  Parameters: $\gamma=40$. $a=0.5,D=0.1,\delta=0.5,k_{2,\max}=1$, $\omega=0.5$. Nutrient input: $\lambda(t)=0.2$.}
\label{fig:autohelp1}
\end{figure}

Next, we consider the following time-periodic nutrient input with some period $T>0$:
\begin{equation}\label{eq:periodic}
\lambda(t)=\begin{cases}0.5,\quad 0\leq t<\frac{T}{2},\\
0,\quad \frac{T}{2}\leq t<T,
\end{cases}
\end{equation}with natural periodic extension to $\mathbb{R^+}$. In the first semi-period, the input of nutrient is relatively sufficient while in the second semi-period period, there is no nutrient input. With this periodic nutrient input, the total density also tends to be periodic, tumor grows in each semi-period with nutrient input, while during the starvation semi-period, population decays. The graphs of total density $n$ at $NT$ (the end of a starvation semi-period) and $NT+\frac{1}{2}T$ (the end of a semi-period with nutrients input), for some $N\in\mathbb{N}$, with the period $T=20$ are shown in Figure \ref{fig:s52perf1}. Here we choose three different $k_{1,\max}$ in three line-styles: solid line for $k_{1,\max}=0$, dashed line for $k_{1,\max}=2$ and dash-dot line for $k_{1,\max}=8$. Each line-style has two curves: the higher one is plotted at $NT+\frac{1}{2}T$, i.e., after a semi-period with nutrient input, and the lower one is plotted at $NT$, i.e., after a starvation semi-period. After a starvation semi-period, the total density is low but the width of ``proliferating rim'' is the same as at the end of a semi-period with nutrient input. If we consider a longer period $T=40$ (Figure \ref{fig:s52perf1long}), the width of tumor after a semi-period with nutrient input is longer, but the density after a starvation period is lower, in particular, one can see when $k_{1,\max}=0$ the population at the end of a starvation semi-period is so low that it can hardly be observed compared to the population at the end of a semi-period with nutrient input.  %Total population is also oscillating in time. If we consider a different growth rate. have smaller oscillation amplitude

Finally, we look at how the total population oscillates with such periodic nutrient input. In Figure \ref{fig:s52perf2}, for all three choices of $k_{1\max}$, the total population $\int_{\Omega}n(x,t)dx$ oscillates periodically with similar amplitudes under the periodic nutrients input. If we extend the model to consider the following logistic type growth rates:
\begin{equation}\label{eq:loggrowth}
G(c,n)=g(M-n)c-\delta,
\end{equation}where  $M>0$ is the carrying capacity and $g>0$. Simulations with \eqref{eq:loggrowth} (Figure \ref{fig:s52logperf2}) show that population with autophagy has a smaller oscillation amplitude than that without autophagy, similar to that in \cite{jin2014mathematical-autophagy}.


\begin{figure}[H]
	\begin{subfigure}{.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{s52perf1}
		\caption{Period $T=20$}
		\label{fig:s52perf1}
	\end{subfigure}
	\begin{subfigure}{.49\linewidth}
			\centering
		\includegraphics[width=0.9\linewidth]{s52perf1long}
		\caption{Period $T=40$}
		\label{fig:s52perf1long}
	\end{subfigure}
		\label{fig:s52period-graph}
		\caption{Plots of the total density $n$ with a periodic nutrient input at the beginning and at the end of the starvation semi-period. Blue solid line: $k_{1,\max}=0$ at $NT+\frac{1}{2}T(N\in\mathbb{N})$. Orange solid line: $k_{1,\max}=0$ at $NT$. Yellow dashed line: $k_{1,\max}=2$ at $NT+\frac{1}{2}T$. Purple dashed line: $k_{1,\max}=2$ at $NT$. Green dash-dot line: $k_{1,\max}=8$ at $NT+\frac{1}{2}T$. Light blue dash-dot line: $k_{1,\max}=8$ at $NT$. Other parameters: $\gamma=40$. $a=0.5,\delta=0.5,D=0.1,k_{2,\max}=1,\omega=0.5$. Nutrient input: \eqref{eq:periodic} with $T=20,40$.}
\end{figure}
\begin{figure}[H]
	\begin{subfigure}{.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{s52perf2}
		\caption{$G(c)=c-\delta$}
		\label{fig:s52perf2}
	\end{subfigure}
	\begin{subfigure}{.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{s52logperf2}
		\caption{$G=G(c,n)=g(M-n)c-\delta$}
		\label{fig:s52logperf2}
	\end{subfigure}
	\label{fig:s52pertime}
	\caption{Evolution of the total population with a time-periodic nutrient input. (a): linear growth rate \eqref{eq:simple-G}. (b): logistic growth rate \eqref{eq:loggrowth}. Solid line: $k_{1,\max}=0$. Dashed line: $k_{1,\max}=2$. Dash-dot line: $k_{1,\max}=8$. Parameters for logistic growth rates: $g=2,M=1.2$. Other parameters: $\gamma=40,a=0.5,\delta=0.5,D=0.1,k_{2,\max}=1$, $\omega=0.5,N_1=N_2=4$.}
\end{figure}


\end{document}

